Filtration and canonical completeness for continuous modal mu-calculi

The continuous modal mu-calculus is a fragment of the modal mu-calculus, where the application of fixpoint operators is restricted to formulas whose functional interpretation is Scott-continuous, rather than merely monotone. By game-theoretic means, we show that this relatively expressive fragment still allows two important techniques of basic modal logic, which notoriously fail for the full modal mu-calculus: filtration and canonical models. In particular, we show that the Filtration Theorem holds for formulas in the language of the continuous modal mu-calculus. As a consequence we obtain the finite model property over a wide range of model classes. Moreover, we show that if a basic modal logic L is canonical and the class of L-frames admits filtration, then the logic obtained by adding continuous fixpoint operators to L is sound and complete with respect to the class of L-frames. This generalises recent results on a strictly weaker fragment of the modal mu-calculus, viz. PDL.

==> eptcsdata.tex <==
\providecommand{\firstpage}{211}
\providecommand{\publicationstatus}{D. Bresolin and P. Ganty (Eds.): 12th International Symposium \\
on Games, Automata, Logics, and Formal Verification (GandALF 2021)\\
EPTCS 346, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.346.14}{10.4204/EPTCS.346.14}}

